LLM4SR: A Survey on Large Language Models for Scientific Research

In recent years, the rapid advancement of Large Language Models (LLMs) has transformed the landscape of scientific research, offering unprecedented support across various stages of the research cycle. This paper presents the first systematic survey dedicated to exploring how LLMs are revolutionizing the scientific research process. We analyze the unique roles LLMs play across four critical stages of research: hypothesis discovery, experiment planning and implementation, scientific writing, and peer reviewing. Our review comprehensively showcases the task-specific methodologies and evaluation benchmarks. By identifying current challenges and proposing future research directions, this survey not only highlights the transformative potential of LLMs, but also aims to inspire and guide researchers and practitioners in leveraging LLMs to advance scientific inquiry. Resources are available at the following repository: https://github.com/du-nlp-lab/LLM4SR

==> 0_related_work.tex <==
% \section{Background and Overview of the Tasks}


==> Tables/3_tools.tex <==
\begin{table}[h!]
\caption{Tools and platforms of scientific research that leverage LLMs for experiment planning and implementation}
\label{tab:exprimental tools}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ll}
\toprule
\textbf{Tools or Platforms} & \textbf{Key Features}                                                                                                                                                                                                                                                                                       & \textbf{Availability} \\ \hline
HuggingGPT\footnotemark~\citep{shen2024hugginggpt}         & \begin{tabular}[c]{@{}l@{}} Decomposes the task into many sub-tasks, and then solves each of them \\ based on models on HuggingFace \end{tabular}& Open source  \\ 
AutoGPT\footnotemark            & \begin{tabular}[c]{@{}l@{}}Autonomously generates hypotheses, designs experiments, allocates resources,\\ executes tasks, adapts in real-time, and provides insights to optimize experimental workflows\end{tabular}                                                                               & Open source  \\ 
AI Scientist\footnotemark~\citep{lu2024ai}       & \begin{tabular}[c]{@{}l@{}}Automates the entire research life cycle, from generating novel research ideas,\\ writing any necessary code, and executing experiments, to summarizing experimental results,\\ visualizing them, and presenting its findings in a full scientific manuscript\end{tabular} & Open source  \\ 
Data to Paper\footnotemark      & \begin{tabular}[c]{@{}l@{}}Perform data exploration, create research hypotheses, conduct literature search, write and \\ debug data analysis code, interpret the results, write the research paper, and backtrack through\\ steps to trace and verify process\end{tabular}                            & Open source  \\ 
GPT Researcher\footnotemark     & \begin{tabular}[c]{@{}l@{}} Develop task-specific questions, trigger web crawls to gather information, summarize sources,\\ and aggregate summaries \end{tabular} & Open source  \\ 
MLR-Copilot\footnotemark~\citep{li2024mlr}        & \begin{tabular}[c]{@{}l@{}}Generate research idea experimental plans, translates experimental plans into executable experiments, \\ run experiments with human feedback and iterative debugging\end{tabular}                                                                                        & Open source  \\ \bottomrule
\end{tabular}
}
\end{table}

\footnotetext[1]{\url{https://huggingface.co/spaces/microsoft/HuggingGPT}}
\footnotetext[2]{\url{https://autogpt.net/}}
\footnotetext[3]{\url{https://github.com/SakanaAI/AI-Scientist}}
\footnotetext[4]{\url{https://github.com/Technion-Kishony-lab/data-to-paper/}}
\footnotetext[5]{\url{https://github.com/assafelovic/gpt-researcher}}
\footnotetext[6]{\url{https://github.com/du-nlp-lab/MLR-Copilot}}

==> Tables/5_tools.tex <==
\begin{table*}[h!]
\centering
\caption{Overview of AI-Powered Academic Research and Review Platforms: Tools supporting both peer review and broader research features}
\label{tab:research_platforms}
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\raggedright\arraybackslash}m{0.15\textwidth}|>{\raggedright\arraybackslash}m{0.45\textwidth}>{\centering\arraybackslash}m{0.25\textwidth}>{\centering\arraybackslash}m{0.15\textwidth}}
\toprule
\textbf{Platform} & \textbf{Additional Key Features} & \textbf{Primary Use Case} & \textbf{Availability} \\
\midrule
SciSpace & 
PDF parsing, reference management, AI writing assistance, journal formatting
& Research Writing & Free / Premium \\
Scite & 
Citation classification, context analysis, network visualization
& Citation Analysis & Free / Premium \\
Semantic Scholar & 
TLDR summaries, citation visualization, paper recommendations
& Literature Discovery & Free \\
Elicit & 
Systematic review automation, study comparison, evidence extraction
& Research Synthesis & Free / Premium \\
Perplexity & 
Real-time web search, information synthesis, source analysis
& Research Assistant & Free / Premium \\
Consensus & 
Claim extraction, evidence synthesis, study comparison
& Evidence Analysis & Free / Premium \\
Scholarcy & 
Paper summarization, flashcard generation, metadata extraction
& Document Analysis & Subscription-based \\
\bottomrule
\end{tabular}}

\end{table*}
